Virtual social science

Can we describe social systems quantitatively and predictively, when we know all the actions, interactions, and states of individuals? We interpret human societies as co-evolutionary systems of individuals and their interactions. Based on unique data of a society of computer game players, where all actions and interactions between all players are known, we show that this might indeed be possible. Within this framework we address a number of sociological classics, including formation of social networks, strength of relations, group formation, hierarchical organization, aggression management, gender differences, mobility, and wealth-inequality. We discover behavioral and organizational patterns of the homo sapiens and its society that were not visible with traditional methodology from the social sciences.

==> references <==

@article{Szell2010msd,
 author           = {Szell, M and Thurner, S},
 title            = {Measuring social dynamics in a massive multiplayer online game},
 journal           = {Social Networks},
 year                = {2010},
 volume          = {32},
 number          = {},
 pages            = {313-329},
 publisher        = {},
 }

@article{Szell2010,
 author               = {M. Szell and R. Lambiotte and S. Thurner},
 journal              = {Proceedings of the National Academy of Sciences},
 number               = {31},
 pages                = {13636-41},
 title                = {Multirelational organization of large-scale social networks in an online world.},
 volume               = {107},
 year                 = {2010},
 }

@ARTICLE{Thurner2012,
  author 		= {Thurner, S and Szell, M  and Sinatra, R}, 
  title 		= {Emergence of good conduct, scaling and Zipf laws in human behavioral sequences in an online world},
  journal 		= {PLoS ONE},
  year 			= {2012},
  volume 		= {7},
  pages 		= {e29796},
  number 		= {1},
}

@article{Szell2012,
 author           = {Szell, M and Sinatra, R and Petri,G and Thurner, S and Latora, V},
 title            = {Understanding mobility in a social petri dish},
 journal          = {Scientific Reports},
 year             = {2012},
 volume           = {2},
 number           = {},
 pages            = {457},
 publisher        = {},
 }
 
@article{Szell2012B,
 author           = {Szell, M and Thurner, S},
 title            = {Social dynamics in a large-scale online game},
 journal          = {Advances in Complex Systems},
 year             = {2012},
 volume           = {15},
 number           = {},
 pages            = {1250064},
 publisher        = {},
 }

@article{Szell2012C,
 author               = {M. Szell and S. Thurner},
 journal              = {Scientific Reports},
 pages                = {01214},
 title                = {How women organize social networks different from men},
 volume               = {3},
 year                 = {2012},
 }

@article{Klimek2013,
 author           = {Klimek, P and Thurner, S},
 title            = {Triadic closure dynamics explains scaling-exponents for preferential attachment-, degree- and clustering distributions in social multiplex data},
 journal          = {New Journal of Physics},
 year             = {2013},
 volume           = {15},
 number           = {},
 pages            = {063008},
 publisher        = {},
 }


@article{CorominasMurtra2014,
 author           = {Corominas-Murtra, B and Hanel, R and Thurner, S},
 title                = {Understanding scaling through history-dependent processes with collapsing sample space},
 journal           = {Proceedings of the National Academy of Sciences},
 year                = {2015},
 volume          = {112},
 number          = {},
 pages            = {5348-5353},
 publisher        = {},
 }

@article{CorominasMurtra2014B,
 author           = {Corominas-Murtra, B and Fuchs, B and Thurner, S},
 title                = {Detection of the elite structure in a virtual multiplex social system by means of a generalized k-core},
 journal           = {PLoS ONE},
 year                = {2014},
 volume          = {9},
 number          = {},
 pages            = {e112606},
 publisher        = {},
 }

@article{Thurner2014,
 author           = {Thurner, S and Fuchs, B},
 title            = {Physical forces between humans? How humans attract and repel each other based on their social interactions in an online world},
 journal          = {PLoS ONE},
 year             = {2014},
 volume           = {10},
 number           = {},
 pages            = {e0133185},
 publisher        = {},
 }
 
@article{Fuchs2014,
 author           = {Fuchs, B and Sornette, D and Thurner, S},
 title            = {Fractal multi-level organisation of human groups in a virtual world},
 journal          = {Scientific Reports},
 year             = {2014},
 volume           = {4},
 number           = {},
 pages            = {6526},
 publisher        = {},
 }

@article{Fuchs2014B,
 author           = {Fuchs, B and  Thurner, S},
 title            = {Behavioral and network origins of wealth inequality: insights from a virtual world},
 journal          = {PLoS ONE},
 year             = {2014},
 volume           = {9},
 number           = {},
 pages            = {e103503},
 publisher        = {},
 }

@article{Mryglod2015,
 author           = {Mryglod, O and  Fuchs, B and Szell, M and Holovatch, Y and Thurner, S},
 title            = {Interevent times of human multi-level activity in a virtual world},
 journal          = {Physica A},
 year             = {2015},
 volume           = {419},
 number           = {},
 pages            = {681-690},
 publisher        = {},
 }

@article{Klimek2016,
 author           = {Klimek, P and Diakonova, M and Egu\'iluz, VM and San Miguel, M and Thurner, S},
 title            = {Dynamical origins of the community structure of an online multi-layer society},
 journal          = {New Journal of Physics},
 year             = {2016},
 volume           = {18},
 number           = {},
 pages            = {083045},
 publisher        = {},
 }

@article{Sadilek2018,
 author           = {Sadilek, M and Klimek, P and Thurner, S},
 title            = {Asocial balance--how your friends determine your enemies: understanding the co-evolution of friendship and enmity interactions in a virtual world},
 journal          = {Journal of Computational Social Science},
 year             = {2018},
 volume           = {1},
 number           = {},
 pages            = {227-239},
 publisher        = {},
 }
 

@book{Wasserman1994,
  title={Social Network Analysis: Methods and Applications},
  author={Wasserman, S and Faust, K},
  volume={8},
  year={1994},
  publisher={Cambridge University Press}
}

@ARTICLE{Granovetter1973,
  author = {Granovetter, M. S.},
  title = {The strength of weak ties},
  journal = {American Journal of Sociology},
  year = {1973},
  volume = {78},
  pages = {1360-1380},
  number = {6},
  file = {},
  owner = {},
  printed = {},
  publisher = {},
  timestamp = {}
}

@BOOK{vonNeumann1944,
   title = {Theory of Games and Economic Behavior},
  publisher = {Princeton University Press},
  year = {1944},
  author = {von Neumann, J and Morgenstern, O},
  address = {New York},
  owner = {},
  timestamp = {}
  }

@ARTICLE{Press2012,
  author = {Press, W.H. and Dyson, F.J.},
  title = {Iterated prisoner's dilemma contains strategies that dominate any evolutionary opponent},
  journal = {Proceedings of the National Academy of Sciences},
  year = {2012},
  volume = {109},
  pages = {10409-10413},
  number = {},
  file = {},
  owner = {},
  printed = {},
  publisher = {},
  timestamp = {}
}


@BOOK{Thurner2018book,
  author = {Thurner, S and Klimek, P and Hanel, R},
  title = {Introduction to the Theory of Complex Systems},
  publisher = {Oxford University Press},
  year = {2018},
  volume = {},
  pages = {},
  number = {},
  file = {},
  owner = {},
  printed = {},
  timestamp = {}
}


@article{Onnela2007PNAS,
 author               = {J.-P. Onnela and J. Saram\"aki and J. Hyv\"onen and G. Szab\'o and D. Lazer and K. Kaski and J. Kert\'esz and A.-L. Barab\'asi},
 journal              = {Proceedings of the National Academy of Sciences},
 number               = {18},
 pages                = {7332-6},
 title                = {Structure and tie strength in mobile communication networks},
 volume               = {104},
 year                 = {2007},

 }


@article{Onnela2007,
 author               = {J.-P. Onnela and J. Saram\"aki and J. Hyv\"onen and G. Szab\'o and M. Argollo de Menezes and K. Kaski and A.-L. Barab\'asi and J. Kert\'esz},
 journal              = {New Journal of Physics},
 pages                = {179},
 title                = {Analysis of large-scale weighted network of one-to-one human communication},
 volume               = {9},
 year                 = {2007},
 }


@article{Kivela2014,
author = {Kivel\"a, M and Arenas, A and Barthelemy, M and Gleeson, J P and Moreno, Y and Porter, M A},
title = {Multilayer networks},
journal = {Journal of Complex Networks},
volume = {2},
number = {3},
pages = {203-271},
year = {2014},
}

@BOOK{Bartle2004,
  title = {Designing virtual worlds},
  publisher = {New Riders Games},
  year = {2004},
  author = {Bartle, R},
  owner = {Michael Szell},
  timestamp = {2009-09-24}
}

@ARTICLE{Castronova2006,
  author = {Castronova, E},
  title = {On the Research Value of Large Games},
  journal = {Games and Culture},
  year = {2006},
  volume = {1},
  pages = {163-186},
  abstract = {Coordination game theory is quite important to a number of literatures
	but has had very few direct empirical tests because that would require
	experimental participation by large numbers of people. Large games
	however can produce natural experiments: situations that through
	no intent of the designer offer controlled variations on a phenomenon
	of theoretical interest. Unlike any other social science research
	technology, such games provide for both sufficient participation
	numbers and careful control of experimental conditions, making them
	like Petri dishes for social science. This article examines two examples
	of games as Petri dishes for macro-level coordination effects: (a)
	the location of markets inside EverQuest and (b) the selection of
	battlefields inside Dark Age of Camelot.},
  owner = {Michael Szell},
  printed = {N},
  timestamp = {2009-09-24}
}

@ARTICLE{Friedkin1980,
  author = {Friedkin, N.},
  title = {A test of structural features of Granovetter's strength of weak ties theory},
  journal = {Social Networks},
  year = {1980},
  volume = {2},
  pages = {411-422},
  number = {4},
  publisher = {Elsevier},
  timestamp = {2009-10-13}
}

@BOOK{Feynman1985,
  author = {Feynman, RP},
  title = {QED: The strange theory of light and matter},
  publisher = {Princeton University Press},
  year = {1985},
  volume = {},
  pages = {},
  number = {},
  file = {},
  owner = {},
  printed = {},
  timestamp = {}
}

@article{Lambiotte2008,
 author           = {Lambiotte, R and Blondel, VD and {de Kerchove}, C and Huens, E and Prieur, C and Smoreda, Z  et~al.},
 title            = {Geographical dispersal of mobile communication networks},
 journal          = {Physica A},
 year             = {2008},
 volume           = {387},
 number           = {21},
 pages            = {5317-5325},
 publisher        = {},
 }


@article{Krings2009,
 author           = {Krings, G and Calabrese, F and Ratti, C and Blondel, VD},
 title            = {Urban gravity: a model for inter-city telecommunication flows},
 journal          = {Journal of Statistical  Mechanics},
 year             = {2009},
 volume           = {7},
 number           = {},
 pages            = {L07003},
 publisher        = {},
 }


@article{Liben-Nowell2005,
 author           = {Liben-Nowell,  D and Novak, J and Kumar, R and  Raghavan, P and Tomkins, A},
 title            = {Geographic routing in social networks},
 journal          = {Proceedings of the National Academy of Sciences},
 year             = {2005},
 volume           = {102},
 number           = {},
 pages            = {11623-11628},
 publisher        = {},
 }



@article{Levy2014,
 author           = {Levy, M and Goldenberg, J},
 title            = {The gravitational law of social interaction},
 journal          = {Physica A},
 year             = {2014},
 volume           = {393},
 number           = {},
 pages            = {418-426},
 publisher        = {},
 }

 
@article{Adamic2005,
 author           = {Adamic, L and Adar, E},
 title            = {How to search a social network},
 journal          = {Social Networks},
 year             = {2005},
 volume           = {27},
 number           = {3},
 pages            = {187-203},
 publisher        = {},
 }

@article{Backstrom2010,
 author           = {Backstrom, L and Sun, E and Marlow, C},
 title            = {Find me if you can: improving geographical prediction with social and spatial proximity},
 journal          = {In: Proceedings of the 19th International Conference on World Wide Web. WWW'10. New York, NY, USA: ACM},
 year             = {2010},
 volume           = {},
 number           = {},
 pages            = {61-70},
 publisher        = {},
 }
 
@article{Scellato2011,
 author           = {Scellato, S and Noulas, A and Lambiotte, R and Mascolo, C},
 title            = {Socio-spatial properties of online location-based social networks},
 journal          = {In: Proceedings of the fifth international AAAI conference on weblogs and social media},
 year             = {2011},
 volume           = {},
 number           = {},
 pages            = {329-336},
 publisher        = {},
 }


@article{Cho2011,
 author           = {Cho, E and Myers, SA and Leskovec, J},
 title            = {Friendship and mobility: user movement in location-based social networks},
 journal          = {In: Proceedings of the 17th ACM SIGKDD international conference on knowledge discovery and data mining. KDD '11. New York, NY, USA: ACM},
 year             = {2011},
 volume           = {},
 number           = {},
 pages            = {1082-1090},
 publisher        = {},
 }


@article{Grabowicz2014,
 author           = {Grabowicz, PA and Ramasco, JJ and Gon\c{c}alves, B and Egu{\'\i}luz, VM},
 title            = {Entangling mobility and interactions in social media},
 journal          = {PLoS ONE},
 year             = {2014},
 volume           = {9},
 number           = {3},
 pages            = {e92196},
 publisher        = {},
 }
 
 
 @article{Davidsen2002,
 author               = {J. Davidsen and H. Ebel and S. Bornholdt},
 journal              = {Physical Review Letters},
 number               = {12},
 pages                = {128701-5},
 title                = {Emergence of a small world from local interactions: modeling acquaintance networks},
 volume               = {88},
 year                 = {2002},
 }


@article{Vazquez2003,
  title={Growing network with local rules: preferential attachment, clustering hierarchy, and degree correlations},
  author={V{\'a}zquez, A},
  journal={Physical Review E},
  volume={67},
  number={5},
  pages={056104},
  year={2003},
  publisher={APS}
}

@article{Holme2002,
 author               = {P. Holme and B.J. Kim},
 journal              = {Physical Review E},
 number               = {2},
 pages                = {026107},
 title                = {Growing scale-free networks with tunable clustering},
 volume               = {65},
 year                 = {2002},
 }

@article{Toivonen2006,
 author               = {Toivonen, R and Onnela, JP and Saram\"aki, J and Hyv\"onen, J and Kaski, K},
 journal              = {Physica A},
 number               = {2},
 pages                = {851-60},
 title                = {A model for social networks},
 volume               = {371},
 year                 = {2006},
 }

@article{Rapoport1953,
 author           = {Rapoport, A},
 title                = {Spread of information through a population with socio-structural bias I: assumption of transitivity},
 journal           = {Bulletin of Mathematical Biophysics},
 year                = {1953},
 volume          = {15},
 number          = {},
 pages            = {523-533},
 publisher        = {},
 }
 

 @article{Jeong2003,
 author               = {H. Jeong and Z. N\'eda and A.-L. Barab\'asi},
 journal              = {Europyhsics Letters},
 number               = {4},
 pages                = {567},
 title                = {Measuring preferential attachment in evolving networks},
 volume               = {61},
 year                 = {2003},
 }

@article{Barabasi1999,
  title={Emergence of scaling in random networks},
  author={Barab{\'a}si, A-L and Albert, R},
  journal={Science},
  volume={286},
  number={5439},
  pages={509-512},
  year={1999},
  publisher={American Association for the Advancement of Science}
}

@article{Newman2001,
 author               = {Newman, MEJ},
 journal              = {Proceedings of the National Academy of Sciences},
 number               = {2},
 pages                = {404-409},
 title                = {The structure of scientific collaboration networks},
 volume               = {98},
 year                 = {2001},
 }

@article{Amaral2000,
 author               = {Amaral, L. A. N.  and Scala, A.  and Barth\'elemy, M.  and Stanley, H.E.},
 journal              = {Proceedings of the National Academy of Sciences},
 number               = {21},
 pages                = {11149-11152},
 title                = {Classes of small-world networks},
 volume               = {97},
 year                 = {2000},
 }


@article{Coleman1988,
 author           = {Coleman, JS},
 title            = {Social capital in the creation of human capital},
 journal          = {American Journal of Sociology},
 year             = {1988},
 volume           = {94},
 number           = {},
 pages            = {95-120},
 publisher        = {},
 }

@ARTICLE{Heider1946,
  author = {Heider, F},
  title = {Attitudes and cognitive organization},
  journal = {Journal of Psychology},
  year = {1946},
  volume = {21},
  pages = {107-112},
  number = {2},
  file = {heider1946aac.pdf:heider1946aac.pdf:PDF},
  owner = {Michael Szell},
  printed = {N},
  timestamp = {2009-01-16}
}

 
 @article{Cartwright1956,
 author           = {Cartwright, D and Harary, F},
 title            = {Structure balance: a generalization of Heider's theory},
 journal          = {Psychological Review},
 year             = {1956},
 volume           = {63},
 number           = {},
 pages            = {277-293},
 publisher        = {},
 }

@article{marvel,
 author           = {Marvel, S and Kleinberg, J and Strogatz, S},
 title            = {The energy landscape of social balance},
 journal          = {Physical Review Letters},
 year             = {2010},
 volume           = {103},
 number           = {},
 pages            = {198701},
 publisher        = {},
 }


@article{Davis1967,
 author           = {Davis, JA},
 title            = {Clustering and structural balance in graphs},
 journal          = {Human Relations},
 year             = {1967},
 volume           = {20},
 number           = {},
 pages            = {181-187},
 publisher        = {},
 }

@article{Antal2006,
 author           = {Antal, T and Krapivsky, P and Redner, S},
 title            = {Social balance on networks: the dynamics of friendship and enmity},
 journal          = {Physica D},
 year             = {2006},
 volume           = {224},
 number           = {},
 pages            = {130-136},
 publisher        = {},
 }

@article{Kumpula2007,
 author           = {Kumpula, J and Onnela, JP and Saram\"aki, J. and  Kaski, K and Kert\'esz, J},
 title            = {Emergence of communities in weighted networks},
 journal          = {Physical Review Letters},
 year             = {2007},
 volume           = {99},
 number           = {},
 pages            = {228701},
 publisher        = {},
 }

@article{Dunbar1995,
 author           = {Dunbar, RIM and Spoors, M},
 title            = {Social networks, support cliques, and kinship},
 journal          = {Human Nature},
 year             = {1995},
 volume           = {6},
 number           = {},
 pages            = {273-290},
 publisher        = {},
 }

@article{Hill2003,
 author           = {Hill, RA and Dunbar, RIM},
 title            = {Social network size in humans},
 journal          = {Human Nature},
 year             = {2003},
 volume           = {14},
 number           = {},
 pages            = {53-72},
 publisher        = {},
 }

@article{Dunbar1993,
 author           = {Dunbar, RIM},
 title            = {Co-evolution of neocortex size, group size and language in humans},
 journal          = {Behavior and Brain Science},
 year             = {1993},
 volume           = {16},
 number           = {},
 pages            = {681-735},
 publisher        = {},
 }


@article{Zhou2005,
 author            = {Zhou, WX and Sornette, D and Hill, RA and Dunbar, RIM},
 title             = {Discrete hierarchical organisation of social group sizes},
 journal           = {Proceedings of the Royal Society B},
 year              = {2005},
 volume            = {272},
 number            = {},
 pages             = {439-444},
 publisher         = {},
 }

@article{Rubinov2010,
 author           = {Rubinov, M and Sporns, O},
 title            = {Complex network measures of brain connectivity: uses and interpretations},
 journal          = {NeuroImage},
 year             = {2010},
 volume           = {52},
 number           = {},
 pages            = {1059-1069},
 publisher        = {},
 }


@article{Hamilton2007,
 author           = {Hamilton, MJ and Milne,  BT and Walker, RS and Burger, O and Brown, JH},
 title            = {The complex structure of hunter-gatherer social networks},
 journal          = {Proceedings of the Royal Society B},
 year             = {2007},
 volume           = {274},
 number           = {},
 pages            = {2195-2202},
 publisher        = {},
 }

@article{Hill2008,
 author           = {Hill, RA and Bentley, RA and Dunbar, RIM},
 title            = {Network scaling reveals consistent fractal pattern in
  hierarchical mammalian societies},
 journal          = {Biological Letters},
 year             = {2008},
 volume           = {4},
 number           = {},
 pages            = {748-751},
 publisher        = {},
 }

@BOOK{Zipf1949,

  title = {Human behavior and the principle of least effort},
  publisher = {Addison-Wesley},
  year = {1949},
  author = {Zipf, G.K.},
  owner = {},
  printed = {N},
  timestamp = {}
}


@ARTICLE{Holyst2011,

  author = {Chmiel, A. and Sienkiewicz, J. and Thelwall, M. and Paltoglou, G. and Buckley, K. and Kappas, A. and Ho{\l}yst, J.A.},
  title = {Collective emotions online and their influence on community life},
  journal = {PloS ONE},
  year = {2011},
  volume = {6},
  pages = {e22207},
  number = {7},
  owner = {},
  publisher = {Public Library of Science},
}


@article{Blondel2008,
  title={Fast unfolding of communities in large networks},
  author={Blondel, Vincent D and Guillaume, Jean-Loup and Lambiotte, Renaud and Lefebvre, Etienne},
  journal={Journal of Statistical Mechanics},
  volume={2008},
  number={10},
  pages={P10008},
  year={2008},
  publisher={IOP Publishing}
}

@ARTICLE{Sinatra2010,
 author = {Sinatra, R. and Condorelli, D. and Latora, V.},
  title = {Networks of motifs from sequences of symbols},
  journal = {Physical Review Letters},
  year = {2010},
  volume = {105},
  pages = {178702},
  number = {17},
}

@ARTICLE{dna,
  author = {Stanley, H.E. and Buldyrev, S.V. and Goldberger, A.L. and Havlin, S. and Peng, C.K. and Simons, M.},
  title = {Scaling features of noncoding {DNA}},
  journal = {Physica A},
  year = {1999},
  volume = {273},
  pages = {1-18},
  number = {1-2},
  owner = {Michael Szell},
  printed = {N},
  publisher = {Elsevier},
  timestamp = {2011-12-15}
}

@ARTICLE{dna2,
  author = {Peng, C.K. and Buldyrev, S.V. and Goldberger, A.L. and Havlin, S. and Sciortino, F. and Simons, M. and Stanley, H.E.},
  title = {Long-range correlations in nucleotide sequences},
  journal = {Nature},
  year = {1992},
  volume = {356},
  pages = {168-170},
  number = {6365},
  file = {peng1992lcn.pdf:peng1992lcn.pdf:PDF},
  owner = {Michael Szell},
  printed = {N},
  timestamp = {2011-12-15}
}

@ARTICLE{dna3,
  author = {Peng, C.K. and Buldyrev, S.V. and Havlin, S. and Simons, M. and Stanley, H.E. and Goldberger, A.L.},
  title = {Mosaic organization of DNA nucleotides},
  journal = {Physical Review E},
  year = {1994},
  volume = {49},
  pages = {1685},
  number = {2},
  owner = {Michael Szell},
  publisher = {APS},
  timestamp = {2011-12-15}
}

@ARTICLE{Hanel2011,
  author = {Hanel, R. and Thurner, S.},
  title = {A comprehensive classification of complex statistical systems and an ab-initio derivation of their entropy and distribution functions},
  journal = {Europhysics Letters},
  year = {2011},
  volume = {93},
  pages = {20006},
  number = {},
  file = {},
  owner = {},
  printed = {},
  timestamp = {}
}

@article{Haythornthwaite2001,
 author           = {Haythornthwaite, C},
 title            = {Exploring multiplexity: social network structures in a computer-supported distance learning class},
 journal          = {The Information Society},
 year             = {2001},
 volume           = {17},
 number           = {},
 pages            = {211},
 publisher        = {},
 }

@article{Grosman2010,
 author           = {Grosman, K},
 title            = {An exploratory study of gender swapping and gender identity in Second Life},
 journal          = {Ph.D. thesis, The Wright Institute},
 year             = {2010},
 volume           = {},
 number           = {},
 pages            = {},
 publisher        = {},
 }


@article{Mcpherson2001,
 author           = {McPherson, M and Smith-Lovin, L and Cook, J},
 title            = {Birds of a feather: homophily in social networks},
 journal          = {Annual Review of Sociology},
 year             = {2001},
 volume           = {},
 number           = {},
 pages            = {415-444},
 publisher        = {},
 }


@article{Yee2007,
 author           = {Yee, N and Bailenson, J},
 title            = {The proteus effect: the effect of transformed self-representation on behavior},
 journal          = {Human Communication Research},
 year             = {2007},
 volume           = {33},
 number           = {},
 pages            = {271-290},
 publisher        = {},
 }


@article{De2006,
 author           = {De~Nood, D and Attema, J},
 title            = {Second life: the second life of virtual reality},
 journal          = {The Hague, EPN-Electronic Highway Platform},
 year             = {2006},
 volume           = {1},
 number           = {},
 pages            = {},
 publisher        = {},
 }


@article{Griffiths2003,
 author           = {Griffiths, M and Davies, M and Chappell, D}, 
 title            = {Breaking the stereotype: the case of online gaming},
 journal          = {CyberPsychology \& Behavior},
 year             = {2003},
 volume           = {6},
 number           = {},
 pages            = {81-91},
 publisher        = {},
 }

@article{Gini1912,
 author           = {Gini, C},
 title            = {Variabilit{\`a} e mutabilit{\`a}},
 journal          = {In: Pizetti E, Salvemini T, editors, Memorie di metodologica statistica, Rome: Libreria Eredi Virgilio Veschi},
 year             = {1912},
 volume           = {},
 number           = {},
 pages            = {},
 publisher        = {},
 }

@article{Dragulescu2001,
 author           = {Dr\u{a}gulescu, A and Yakovenko, VM},
 title            = {Exponential and power-law probability distributions of wealth and income in the {U}nited {K}ingdom and the {U}nited {S}tates},
 journal          = {Physica A},
 year             = {2001},
 volume           = {299},
 number           = {},
 pages            = {213-221},
 publisher        = {},
 }


@article{Barabasi2005,
 author           = {Barab\'asi, A.-L.},
 title            = {The origin of bursts and heavy tails in humans dynamics},
 journal          = {Nature},
 year             = {2005},
 volume           = {435},
 number           = {},
 pages            = {207},
 publisher        = {},
 }

@article{Sinatra2010nms,
 author           = {Sinatra, R and Condorelli, D and Latora, V},
 title            = {Networks of motifs from sequences of symbols},
 journal          = {Physical Review Letters},
 year             = {2010},
 volume           = {105},
 number           = {},
 pages            = {178702},
 publisher        = {},
 }

@article{Bazzani2010,
 author           = {Bazzani, A and Giorgini, B and Rambaldi, S and Gallotti, R and Giovannini, L},
 title            = {Statistical laws in urban mobility from microscopic gps data in the area of florence},
 journal          = {Journal of Statistical Mechanics},
 year             = {2010},
 volume           = {10},
 number           = {},
 pages            = {P05001},
 publisher        = {},
 }


@article{Roth2010,
 author           = {Roth, C and Kang, SM and Batty, M and Barth{\'e}lemy, M},
 title            = {Structure of urban movements: polycentric activity
  and entangled hierarchical flows},
 journal          = {PLoS ONE},
 year             = {2011},
 volume           = {6},
 number           = {},
 pages            = {e15923},
 publisher        = {},
 }

@article{Song2010,
 author           = {Song, C and Koren, T and Wang, P. and Barab\'asi, A.-L.},
 title            = {Modelling the scaling properties of human mobility},
 journal          = {Nature Physics},
 year             = {2010},
 volume           = {6},
 number           = {},
 pages            = {818-823},
 publisher        = {},
 }
 
 @article{Barthelemy2010,
 author           = {Barth{\'e}lemy, M},
 title            = {Spatial networks},
 journal          = {Physics Reports},
 year             = {2010},
 volume           = {499},
 number           = {},
 pages            = {036113},
 publisher        = {1-101},
 }


@article{Brockmann2006,
 author           = {Brockmann, D and Hufnagel, L and Geisel, T},
 title            = {The scaling laws of human travel},
 journal          = {Nature},
 year             = {2006},
 volume           = {439},
 number           = {},
 pages            = {462-465},
 publisher        = {},
 }
 
@book{Castronova2005,
 address              = {Chicago},
 author               = {Castronova E},
 publisher            = {University of Chicago Press},
 timestamp            = {2009-09-24},
 title                = {Synthetic Worlds: The Business and Culture of Online Games},
 year                 = {2005},
 }

